Don't sweat the small stuff, classify the rest: Sample Shielding to protect text classifiers against adversarial attacks

Deep learning (DL) is being used extensively for text classification. However, researchers have demonstrated the vulnerability of such classifiers to adversarial attacks. Attackers modify the text in a way which misleads the classifier while keeping the original meaning close to intact. State-of-the-art (SOTA) attack algorithms follow the general principle of making minimal changes to the text so as to not jeopardize semantics. Taking advantage of this we propose a novel and intuitive defense strategy called Sample Shielding. It is attacker and classifier agnostic, does not require any reconfiguration of the classifier or external resources and is simple to implement. Essentially, we sample subsets of the input text, classify them and summarize these into a final decision. We shield three popular DL text classifiers with Sample Shielding, test their resilience against four SOTA attackers across three datasets in a realistic threat setting. Even when given the advantage of knowing about our shielding strategy the adversary's attack success rate is <=10% with only one exception and often < 5%. Additionally, Sample Shielding maintains near original accuracy when applied to original texts. Crucially, we show that the `make minimal changes' approach of SOTA attackers leads to critical vulnerabilities that can be defended against with an intuitive sampling strategy.

==> graveyard.tex <==
\vspace{-0.1in}
\subsection{Attack against model protected by Sample Shielding}
\vspace{-0.05in}
\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{shielded_model.pdf}
    \caption{Visualization of main results (solid box) where attacker gets feedback from the classifier and perturbed text is passed to Sample Shielding, and attack where Sample Shielding is incorporated into the classifier (dotted box), which gives feedback to the Attacker. The perturbed text is given to the same model. }
    \label{fig:shieldAttack}
\end{figure}

Our main results focus on attacks against unshielded classifiers.  Here we ask: what happens when the attacks are against classifier models protected with \textit{Sample Shielding}?
Figure \ref{fig:shieldAttack} visualizes the difference between the threat models. In the original scenario (solid box), the attacker uses feedback from the base classifier to craft a perturbed text which it believes will fool the classifier. Then \textit{Sample Shielding} is applied when classifying the perturbed text. For the current experiment (dotted box), the attacker receives feedback from a classifier which already leverages \textit{Sample Shielding}. Once again, the attacker crafts perturbed text which it believes will fool this shielded classifier. When the perturbed text is given to the shielded classifier it again samples the text and aggregates the decision using majority vote --- consistent with its \textit{Sample Shielding} defense.

%We measure accuracy and the average number of queries that the attacker makes to the classifier during the attack. Larger numbers indicate greater effort for the attacker. 
We run this experiment on a subset of 200 examples from the IMDB dataset. We test Textfooler against both LSTM and BERT. Word Sampling with a $p=0.3$ and $k=100$ is used for both. The results are in Table \ref{tab:adversarial}. 
The table shows two blocks of results one where the classifier is not shielded and the second with the shielded classifier.

%This design is unique across defense papers in that we see an example of a shielding technique which is led onto the classifier as well as used during deployment.


\begin{table*}[]
    \centering
    \small
    \begin{tabular}{c||c|c|c|c||c|c|c|c|}
        & \multicolumn{4}{|c||}{Non Shielded} & \multicolumn{4}{|c|}{Shielded}\\\hline
          & Orig. & Attack & Shield & \#  & Orig. & \textit{Acc. Believed} & Attack & \# \\
         Classifier &  Acc.  & Acc. & Acc. & Queries & Acc. & \textit{by attacker} & Acc. & Queries \\\hline
         LSTM & 90.5 & 0.0 & 65.0 & 315.38 &  85.5 & \textit{7.0} & 72.5 & 924.99\\\hline
         BERT & 93.0 & 1.0 & 77.0 & 626.87 & 81.1 & \textit{14.0} & 73.0 & 927.02\\\hline
    \end{tabular}
    \caption{Results of attack of classifier with and without protection of \textit{Sample Shielding}. Orig. Acc. and  Attack Acc. are the accuracy of the classifier against original and attacked texts. Shield Acc. is the accuracy after applying Sample Shielding. \# Queries is the number of queries used by Textfooler against a classifier. Acc. Believed by attacker is the accuracy the attacker believes the perturbed text will cause the classifier to get.}
    \label{tab:adversarial}
\end{table*}


\noindent \textbf{Sample Shielding resists attacks and increases queries.} As before the attack is very successful on the unshielded classifier - accuracies are close to 0.  Also as before, shielding brings large improvements to accuracy. When the classifier is shielded with \textit{Sample Shielding}, original accuracies drop some. During the attack, the attacker uses feedback from the shielded classifier and perturbs a text until it either successfully misleads the classifier or it gives up on the text.  At this point the accuracies believed by the attacker are 7.0 and 14.0 for LSTM and BERT respectively.  However, once these perturbed texts are given back to the protected classifiers to be classified, fresh samples of the perturbed text are taken in line with \textit{Sample Shielding} and accuracy returns to a high of 73\%. 
%[[This is surprising to the attacker as they crafted texts which they believed would fool the classifier.]]
It is precisely due to randomness in sampling that the defense strategy remains successful and the classifier resilient. %These are striking results as it means an attacker cannot rely on the classifier failing against previously attacked text????.

Additionally, the number of queries Textfooler needs to complete attacks is increased greatly. For LSTM, it is increased from 315 on average to 925. For BERT, it is increased from 627 to 927. Both demonstrate additional problems for the attacker especially if it is constrained by the number of queries it can make. 

\noindent\textbf{Comparisons to other attacks.} \citet{Li2021SearchingFA} compare various defenses on an IMDB subset against Textfooler. Though the IMDB set is not the exact same, we can make some observations which can be further tested in future work. First, the accuracy for the top defense \cite{Li2021SearchingFA} is 45.3. Our 73.0 is a large improvement over this.  Second, inline with other strong defenses, \textit{Sample Shielding} causes a large increase in the number of queries needed by the attacker. These beginning insights should be further explored by testing the methods on the exact same subset in the future.



\begin{table*}[]
    \centering
    \footnotesize
    \begin{tabular}{c||c||c|c||c|c||c|c||c|c||c|c}
        & & Sample & Orig. & \multicolumn{2}{|c|}{Textfooler} & \multicolumn{2}{|c|}{Bert-Attack} & \multicolumn{2}{|c|}{TextBugger} & \multicolumn{2}{|c}{PWWS} \\
         & Classifier & Strategy & Acc. & Acc. & ASR  & Acc. & ASR & Acc. & ASR & Acc.  & ASR \\\hline
         \parbox[t]{2mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{IMDB}}}  &  \multirow{3}{*}{LSTM} & Unsampled  & 91	& 0 & 100 & 0 & 100 &	0 & 100 & 0 & 100 \\
         & & Local (W') Word & 87 &	11 & 87	& 31 & 64	& 28 & 68 & 22 & 75\\
         & & Website (W) Word & 94 & \textbf{89} & \textbf{5}	& \textbf{87} & \textbf{7}	& \textbf{89} & \textbf{5} & \textbf{89} & \textbf{5} \\\cline{2-12}
         
         & \multirow{3}{*}{CNN} & Unsampled  & 86 & 0 & 100 & 0 & 100 & 0 & 100 & 0 & 100 \\
         & & Local (W') Word & 91 & 22 & 76	& 22 & 76	& 32 & 65 & 29 & 68\\
         & & Website (W) Word & 89	& \textbf{88} & \textbf{1}	& \textbf{88} & \textbf{1} & \textbf{89} & \textbf{0} & \textbf{86} & \textbf{3}\\\cline{2-12}
         
         & \multirow{3}{*}{BERT} & Unsampled  & 90 & 1 & 99	& 4	& 96 & 6 & 93 & 2 & 98\\
         & & Local (W') Word & 81 & 18 & 78	& 31 & 62	& 34 & 58 & 26 & 68\\
         & & Website (W) Word & 85 & \textbf{80}	& \textbf{6} & \textbf{80} & \textbf{6} & \textbf{84} & \textbf{1} & \textbf{82} & \textbf{4}\\\hline 
         
         % YELP
          \parbox[t]{2mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{Yelp}}}  & \multirow{3}{*}{LSTM} & Unsampled  & 95 & 0 & 100 & 0 & 100 & 6 & 94 & 0 & 100\\
         & & Local (W') Word & 90 & 32 & 64 & 29 & 68 & 44 & 51 & 34& 62 \\
         & & Website (W) Word & \textbf{87} & \textbf{81} & \textbf{7} & \textbf{79} & \textbf{9} & \textbf{78} & \textbf{10} & \textbf{74} & \textbf{15}\\\cline{2-12}
         
         & \multirow{3}{*}{CNN} & Unsampled  & 96 & 0 & 100 & 0 & 100 & 5 & 95 & 3 & 97\\
         & & Local (W') Word & 86 & 36 & 58 & 28 & 67	& 44 & 49 &	40 & 53 \\
         & & Website (W) Word & 88	& \textbf{85} & \textbf{3} & \textbf{81} & \textbf{8} & \textbf{81} & \textbf{8} & \textbf{83} & \textbf{6} \\\cline{2-12}
         
         & \multirow{3}{*}{BERT} & Unsampled  & 100	& 3	& 97 & 10 & 90 & 13 & 87 &7 & 93\\
         & & Local (W') Word & 93 & 40 & 57 & 34 & 63 & 51 & 45 & 50 & 46\\
         & & Website (W) Word & 92 & \textbf{90}	& \textbf{2} & \textbf{88} & \textbf{4}	& \textbf{91} & \textbf{1} & \textbf{85} & \textbf{8} \\\hline 
         
         
         %AG News
          \parbox[t]{2mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{AG News}}} 
         & \multirow{3}{*}{LSTM} & Unsampled  & 93 &	1 & 99 & 0 & 100 & 16 & 83 & 13 & 86 \\
         & & Local (W') Word & 88 & 42 & 52 & 31 & 65	& 38 & 57 & 55 & 38
         \\
         & & Website (W) Word & \textbf{87} & \textbf{78} & \textbf{10}	& \textbf{84} & \textbf{3} & \textbf{78} & \textbf{10} & \textbf{84} & \textbf{3}\\\cline{2-12}
         
         & \multirow{3}{*}{CNN} & Unsampled  & 92 &	1 & 99 & 0 & 100 & 7 & 92 & 3 & 97\\
         & & Local (W') Word & 86 & 45 & 48 & 28 & 67	& 36 & 58 & 54 & 37
         \\
         & & Website (W) Word & 87	& \textbf{81} & \textbf{7}	& \textbf{87} & \textbf{0} & \textbf{84} & \textbf{3} & \textbf{83} & \textbf{5}
         \\\cline{2-12} 
         
         & \multirow{3}{*}{BERT} & Unsampled  & 99 & 20 & 78 & 11 & 89 & 60 & 39 & 15 & 85 \\
         & & Local (W') Word & 88 & 48 & 45	& 38 & 57	& 55 & 38 & 64 & 27\\
         & & Website (W) Word & 88	& \textbf{81} & \textbf{8} & \textbf{82} & \textbf{7} &\textbf{83} & \textbf{6} & \textbf{85} & \textbf{3} \\\hline 
         
    \end{tabular}
    \caption{Results of attack with local knowledge of Sample Shielding. For all shielding cases, $k=30$, $p=0.3$, and majority voting is used. Acc. is accuracy, and ASR is success rate of attack (\%) and Orig. Acc. is accuracy on the original text.}
    \label{tab:adversarialResults}
\end{table*}





\begin{table*}[]
    \centering
    \footnotesize
    \begin{tabular}{c||c||c|c||c|c||c|c||c|c||c|c}
        & & Sampling & Orig. & \multicolumn{2}{|c|}{TextFooler} & \multicolumn{2}{|c|}{Bert-Attack} & \multicolumn{2}{|c|}{TextBugger} & \multicolumn{2}{|c}{PWWS} \\
         & Classifier & Strategy & Acc. & Acc. & SR  & Acc. & SR & Acc. & SR & Acc.  & SR \\\hline
         \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{IMDB}}}  &
         \multirow{4}{*}{LSTM} & No Shielding&  88.3 & 0 & 100 & 0 & 100  & 0.3 & 100 & 0.1 & 100\\
         & & Maj. Vot. & 85.1  & \textbf{66.0} & \textbf{25} & 67.0 & 24 & 66.0 & \textbf{25} & 65.7 & 26
         \\
        & & NN & 85.3 & 62.5 & 29 & 62.1 & 30  & 65.4 & 26 & 62.4 & 29\\
        & & NN-BB & 85.3 & 65.2 & 26 & \textbf{68.2} & \textbf{23} & \textbf{66.5} & \textbf{25} & \textbf{67.3} & \textbf{24} \\\cline{2-12}
        
        
        
         & \multirow{4}{*}{CNN} & No Shielding &  86.2 & 0.1 & 100 & 0 & 100 & 0.3 & 100 & 0 & 100 \\
         & & Maj. Vot. & 84.7 &  \textbf{69.8} &  \textbf{19} & 66.7 & 23 & 71.6 & 17 & 67.8 & 21\\
         & & NN & 84.8 & 61.7 & 28 & 59.6 & 31 & 66.7 & 23 &  60.0 & 30 \\
         & & NN-BB & 84.8 & 69.3 & 20 &  \textbf{67.9} &  \textbf{21} & \textbf{72.3} & \textbf{16} & \textbf{69.6} & \textbf{19} \\\hline
         
        % & \multirow{3}{*}{BERT} & No Shielding & 91.3 & 1 &  3.7 & 9.2 &  \\
        % & & Shielding-Word & 86.8 & 74.4 & 71.5 & &\\ 
       %  & & NN & & & & &          \\\hline
         
         
         
         % YELP
         \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Yelp}}}  & \multirow{4}{*}{LSTM} & No Shielding &  92.5 & 0.3 & 100 &  0.7 & 99 & 5 & 95 & 1.5 & 98 \\
         & & Maj. Vot. & 87.8 & 65.5 & 29 & 66.7 & 28 & 68.5 & 26 & 61.9 & 33 \\
         & & NN & 89.0 & 68.7 & 26 & 68.1 & 26 &  \textbf{73.5} &  \textbf{21} & 63.6 & 31 \\
        & & NN-BB & 89 & \textbf{69.7} & \textbf{25} & \textbf{70.0} & \textbf{24} &   \textbf{73.5} &   \textbf{21} & \textbf{64.9} & \textbf{30} \\\cline{2-12}
           
         & \multirow{4}{*}{CNN} & No Shielding & 94.1 & 0.8 & 99 & 0.4 & 100 & 5.5 & 94 & 2.4 & 97\\
         & & Maj. Vot. & 88.1 & 64.9 & 31 & 62.2 & 34 & 70.4 & 25 & 60.2 & 36 \\
         & & NN & 89.9 & 63.2 & 33 & 57.6 & 39 & 69.9 & 26 & 57.4 & 39\\
         & & NN-BB & 89.9 & \textbf{72.2} & \textbf{23} & \textbf{69.7} & \textbf{26} & \textbf{72.9} & \textbf{23} &   \textbf{67.6} &   \textbf{28} \\\hline
         
         %& \multirow{3}{*}{BERT} & No Shielding & 100 & 5.9 & 8.3 & 15.5 & \\
         %& & Shielding-Word & 93.5 & 69.9 & 75.1 & & \\
        % & & NN & & & & & \\         \hline
         
     
         
    \end{tabular}
    \caption{Comparing vote summarizers. Settings: $k=100$, $p=0.3$, word sampling. Maj. Vot: majority voting, NN: neural network trained on original texts, NN-BB: neural network trained on original + perturbed texts.}
    \label{tab:secondaryResults}
\end{table*}

